Most Expected Winner: An Interpretation of Winners over Uncertain Voter Preferences

It remains an open question how to determine the winner of an election when voter preferences are incomplete or uncertain. One option is to assume some probability space over the voting profile and select the Most Probable Winner (MPW) -- the candidate or candidates with the best chance of winning. In this paper, we propose an alternative winner interpretation, selecting the Most Expected Winner (MEW) according to the expected performance of the candidates. We separate the uncertainty in voter preferences into the generation step and the observation step, which gives rise to a unified voting profile combining both incomplete and probabilistic voting profiles. We use this framework to establish the theoretical hardness of \mew over incomplete voter preferences, and then identify a collection of tractable cases for a variety of voting profiles, including those based on the popular Repeated Insertion Model (RIM) and its special case, the Mallows model. We develop solvers customized for various voter preference types to quantify the candidate performance for the individual voters, and propose a pruning strategy that optimizes computation. The performance of the proposed solvers and pruning strategy is evaluated extensively on real and synthetic benchmarks, showing that our methods are practical.

==> tex/approx.tex <==
\section{Approximate solvers}
\label{sec:approx}

Since the \esc problem over partial voting profiles are proved to be intractable in Section~\ref{sec:complexity}, we now propose a sampling-based estimator for these voting profiles, and more generally, the ones of Mallows models combined with partial orders.
This estimator relies on Theorem~\ref{theorem:reduction} and aims to solve the REP over a Mallows model $\mallows(\bsigma, \phi)$ combined with a partial order $\partialOrder$.
The partial voting profiles are a special case where the Mallows models are uniform distributions with the spread parameter $\phi=1$.

\paragraph{Problem formalization.}
Given a Mallows model $\mallows(\bsigma, \phi)$ of $m$ items, a partial order $\partialOrder$, a rank $1 \leq k \leq m$ and a candidate $c$, we are interested in $\Pr(c \rightarrow k \mid \bsigma, \phi, \partialOrder)$, the probability that candidate $c$ is placed at rank $k$ by a ranking drawn from the posterior distribution of $\mallows(\bsigma, \phi)$ conditioned on $\partialOrder$.

The difficult part of this problem origins from the fact that there is no efficient exact sampling method for the Mallows posteriors conditioned on the partial orders. We can easily come up with a rejection sampler (RS) to draw rankings from $\mallows(\bsigma, \phi)$ and only accept the samples that are the completions of the partial order $\partialOrder$. But this sampler is inept when the posterior probability of the partial order is low enough that samples are almost always rejected.  Importance Sampling (IS) can tackle this issue; it effectively estimates rare events by obtaining samples from an proposal distribution then re-weight the samples for unbiased estimation~\cite{kahn1950random1, kahn1950random2}.

Assume that IS draws $N$ samples $\set{x_1, \ldots, x_N}$ from a proposal distribution $\propDistr$ to estimate the expected value of a function $f(x)$ in a probability space $\oriDistr$.

\begin{equation}\label{eq:importance_sampling}
\small 
\begin{split}
  \mathds{E}(f(x)) 
  =& \sum_{x \in \oriDistr} {f(x) \cdot \Pr(x \mid \oriDistr)} 
  = \sum_{x \in \propDistr} {f(x) \cdot \frac{\Pr(x \mid \oriDistr)}{\Pr(x \mid \propDistr)} \cdot \Pr(x \mid \propDistr)} \\
  =& \mathds{E}\left( f(x) \cdot \frac{\Pr(x \mid \oriDistr)}{\Pr(x \mid \propDistr)} \right)
  \approx \frac{1}{N} \sum_{i=1}^{N} {f(x_i) \cdot \frac{\Pr(x_i \mid \oriDistr)}{\Pr(x_i \mid \propDistr)}}
\end{split}
\end{equation}

IS re-weights the contribution of $x_i$ by an \e{importance factor} $\frac{\Pr(x_i \mid \oriDistr)}{\Pr(x_i \mid \propDistr)}$.
An ideal $\propDistr$ should be easy to draw samples from and be similar to the real posterior distribution.
When applying IS, we adopt AMP, the state-of-the-art Mallows posterior sampler~\cite{DBLP:journals/jmlr/LuB14}, and $f(x_i) = \mathds{1}(c {\rightarrow} k \mid x_i)$, \ie whether candidate $c$ is placed at rank $k$ by sample ranking $x_i$.

